Modeling Populations of Thermostatic Loads with Switching Rate Actuation

We model thermostatic devices using a stochastic hybrid description, and introduce an external actuation mechanism that creates random switch events in the discrete dynamics. We then conjecture the form of the Fokker-Planck equation and successfully verify it numerically using Monte Carlo simulations. The actuation mechanism and subsequent modeling result are relevant for power system operation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{13}
\providecommand{\publicationstatus}{M. Bujorianu (Ed.) and R. Wisniewski (Ed.): 4th Workshop on\\ Hybrid Autonomous Systems 2014 (HAS 2014).\\
EPTCS 174, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.174.2}{10.4204/EPTCS.174.2}}
\pdfoutput=1

